Results from a Prototype Chicane-Based Energy Spectrometer for a Linear Collider

The International Linear Collider and other proposed high energy e+ e- machines aim to measure with unprecedented precision Standard Model quantities and new, not yet discovered phenomena. One of the main requirements for achieving this goal is a measurement of the incident beam energy with an uncertainty close to 1e-4. This article presents the analysis of data from a prototype energy spectrometer commissioned in 2006--2007 in SLAC's End Station A beamline. The prototype was a 4-magnet chicane equipped with beam position monitors measuring small changes of the beam orbit through the chicane at different beam energies. A single bunch energy resolution close to 5e-4 was measured, which is satisfactory for most scenarios. We also report on the operational experience with the chicane-based spectrometer and suggest ways of improving its performance.

==> commands.tex <==
%% Define some useful new commands
%% --------------------------

\newcommand{\ns}{\ensuremath{~\rm{ns}}}
\newcommand{\us}{\ensuremath{~\rm{\mu s}}}
\newcommand{\ms}{\ensuremath{~\rm{ms}}}

\newcommand{\m}{\ensuremath{~\rm{m}}}
\newcommand{\mm}{\ensuremath{~\rm{mm}}}
\newcommand{\um}{\ensuremath{~\rm{\mu m}}}
\newcommand{\nm}{\ensuremath{~\rm{nm}}}

\newcommand{\GeV}{\ensuremath{~\rm{GeV}}}
\newcommand{\MeV}{\ensuremath{~\rm{MeV}}}
\newcommand{\keV}{\ensuremath{~\rm{keV}}}

\newcommand{\GHz}{\ensuremath{~\rm{GHz}}}
\newcommand{\MHz}{\ensuremath{~\rm{MHz}}}
\newcommand{\kHz}{\ensuremath{~\rm{kHz}}}
\newcommand{\Hz}{\ensuremath{~\rm{Hz}}}

\newcommand{\dB}{\ensuremath{~\rm{dB}}}
\newcommand{\dBm}{\ensuremath{~\rm{dBm}}}

\newcommand{\E}[1]{\ensuremath{\times 10^{#1}}}

\newcommand{\rad}{\ensuremath{~\rm{rad}}}
\newcommand{\mrad}{\ensuremath{~\rm{mrad}}}
\newcommand{\urad}{\ensuremath{~\mu \rm{rad}}}

\newcommand{\degA}{\ensuremath{^{\circ}}}
\newcommand{\degC}{\ensuremath{^{\circ} {\rm C}}}

